Emergent Abilities in Reduced-Scale Generative Language Models

Large language models can solve new tasks without task-specific fine-tuning. This ability, also known as in-context learning (ICL), is considered an emergent ability and is primarily seen in large language models with billions of parameters. This study investigates if such emergent properties are strictly tied to model size or can be demonstrated by smaller models trained on reduced-scale data. To explore this, we simplify pre-training data and pre-train 36 causal language models with parameters varying from 1 million to 165 million parameters. We show that models trained on this simplified pre-training data demonstrate enhanced zero-shot capabilities across various tasks in simplified language, achieving performance comparable to that of pre-trained models six times larger on unrestricted language. This suggests that downscaling the language allows zero-shot learning capabilities to emerge in models with limited size. Additionally, we find that these smaller models pre-trained on simplified data demonstrate a power law relationship between the evaluation loss and the three scaling factors: compute, dataset size, and model size.

==> tables/table_blimp_filtered_limited.tex <==
% blimp filtered results on few benchmarks only
\begin{table*}[h!]
\begin{tabularx}{\textwidth}{XXXXXXXXXXXXXXX}
\toprule
Hidden & Num. & Aanphor & Control/  & Ellipsis &                          Avg. \\
Size & Layers & Agreement & Raising & &                          Score \\
\midrule
       1024 &           8 &  0.968 $\textcolor{green}{\uparrow}$ &  0.792 $\textcolor{green}{\uparrow}$ &  0.806 $\textcolor{green}{\uparrow}$ &  0.794 $\textcolor{green}{\uparrow}$ \\
       1024 &           8 &                                0.958 &                                0.775 &                                0.722 &                                0.768 \\
       1024 &           4 &  0.965 $\textcolor{green}{\uparrow}$ &  0.766 $\textcolor{green}{\uparrow}$ &  0.781 $\textcolor{green}{\uparrow}$ &  0.772 $\textcolor{green}{\uparrow}$ \\
       1024 &           4 &                                0.951 &                                0.755 &                                0.721 &                                0.748 \\
       1024 &           2 &  0.961 $\textcolor{green}{\uparrow}$ &  0.778 $\textcolor{green}{\uparrow}$ &  0.736 $\textcolor{green}{\uparrow}$ &  0.769 $\textcolor{green}{\uparrow}$ \\
       1024 &           2 &                                0.927 &                                0.729 &                                0.689 &                                 0.74 \\
        512 &           8 &  0.938 $\textcolor{red}{\downarrow}$ &  0.762 $\textcolor{green}{\uparrow}$ &  0.761 $\textcolor{green}{\uparrow}$ &  0.767 $\textcolor{green}{\uparrow}$ \\
        512 &           8 &                                0.952 &                                0.745 &                                 0.66 &                                0.746 \\
        512 &           4 &  0.961 $\textcolor{green}{\uparrow}$ &  0.779 $\textcolor{green}{\uparrow}$ &  0.757 $\textcolor{green}{\uparrow}$ &  0.771 $\textcolor{green}{\uparrow}$ \\
        512 &           4 &                                0.938 &                                0.748 &                                0.654 &                                0.742 \\
        512 &           2 &  0.915 $\textcolor{green}{\uparrow}$ &  0.763 $\textcolor{green}{\uparrow}$ &  0.744 $\textcolor{green}{\uparrow}$ &  0.749 $\textcolor{green}{\uparrow}$ \\
        512 &           2 &                                 0.88 &                                0.736 &                                0.679 &                                0.721 \\
        256 &           8 &  0.913 $\textcolor{green}{\uparrow}$ &  0.761 $\textcolor{green}{\uparrow}$ &  0.656 $\textcolor{green}{\uparrow}$ &  0.732 $\textcolor{green}{\uparrow}$ \\
        256 &           8 &                                0.897 &                                0.749 &                                0.626 &                                0.723 \\
        256 &           4 &  0.936 $\textcolor{green}{\uparrow}$ &  0.772 $\textcolor{green}{\uparrow}$ &   0.67 $\textcolor{green}{\uparrow}$ &  0.744 $\textcolor{green}{\uparrow}$ \\
        256 &           4 &                                0.867 &                                0.715 &                                0.617 &                                0.715 \\
        256 &           2 &  0.893 $\textcolor{green}{\uparrow}$ &  0.749 $\textcolor{green}{\uparrow}$ &  0.674 $\textcolor{green}{\uparrow}$ &  0.724 $\textcolor{green}{\uparrow}$ \\
        256 &           2 &                                0.798 &                                0.718 &                                0.605 &                                0.697 \\
        128 &           8 &  0.884 $\textcolor{green}{\uparrow}$ &  0.761 $\textcolor{green}{\uparrow}$ &  0.654 $\textcolor{green}{\uparrow}$ &  0.729 $\textcolor{green}{\uparrow}$ \\
        128 &           8 &                                0.785 &                                0.731 &                                0.591 &                                0.685 \\
        128 &           4 &  0.854 $\textcolor{green}{\uparrow}$ &  0.754 $\textcolor{green}{\uparrow}$ &  0.624 $\textcolor{red}{\downarrow}$ &  0.717 $\textcolor{green}{\uparrow}$ \\
        128 &           4 &                                0.774 &                                0.703 &                                0.632 &                                0.697 \\
        128 &           2 &  0.847 $\textcolor{green}{\uparrow}$ &  0.756 $\textcolor{green}{\uparrow}$ &  0.675 $\textcolor{green}{\uparrow}$ &  0.711 $\textcolor{green}{\uparrow}$ \\
        128 &           2 &                                0.802 &                                0.673 &                                0.593 &                                0.669 \\
         64 &           8 &  0.847 $\textcolor{green}{\uparrow}$ &  0.692 $\textcolor{green}{\uparrow}$ &  0.575 $\textcolor{green}{\uparrow}$ &  0.707 $\textcolor{green}{\uparrow}$ \\
         64 &           8 &                                0.696 &                                 0.69 &                                0.543 &                                0.646 \\
         64 &           4 &  0.807 $\textcolor{green}{\uparrow}$ &  0.699 $\textcolor{green}{\uparrow}$ &  0.556 $\textcolor{red}{\downarrow}$ &  0.673 $\textcolor{green}{\uparrow}$ \\
         64 &           4 &                                0.697 &                                0.656 &                                0.588 &                                0.646 \\
         64 &           2 &   0.79 $\textcolor{green}{\uparrow}$ &  0.683 $\textcolor{green}{\uparrow}$ &  0.577 $\textcolor{red}{\downarrow}$ &  0.667 $\textcolor{green}{\uparrow}$ \\
         64 &           2 &                                0.637 &                                0.623 &                                0.596 &                                0.628 \\
         32 &           8 &  0.746 $\textcolor{red}{\downarrow}$ &  0.632 $\textcolor{green}{\uparrow}$ &  0.498 $\textcolor{red}{\downarrow}$ &  0.641 $\textcolor{green}{\uparrow}$ \\
         32 &           8 &                                0.762 &                                0.589 &                                0.521 &                                0.629 \\
         32 &           4 &  0.479 $\textcolor{red}{\downarrow}$ &  0.644 $\textcolor{green}{\uparrow}$ &  0.489 $\textcolor{green}{\uparrow}$ &  0.599 $\textcolor{red}{\downarrow}$ \\
         32 &           4 &                                0.612 &                                0.609 &                                0.488 &                                0.614 \\
         32 &           2 &  0.723 $\textcolor{green}{\uparrow}$ &  0.631 $\textcolor{green}{\uparrow}$ &  0.485 $\textcolor{green}{\uparrow}$ &   0.64 $\textcolor{green}{\uparrow}$ \\
         32 &           2 &                                0.591 &                                0.626 &                                 0.42 &                                0.584 \\
\bottomrule
\end{tabularx}
\caption{Zero-shot accuracy scores on the vocabulary filtered datasets on the BLiMP benchmark. For each hidden layer size and layer count, the table compares metrics for both simple and regular models.  The initial row for each hidden size and number of layers displays results from the simple model trained on simplified data, followed by a similar-sized regular model trained on regular data. Performance comparison is indicated by arrows next to the simple model's scores: a $\textcolor{green}{\uparrow}$ signifies the simple model outperforming the regular model, while a $\textcolor{red}{\downarrow}$ denotes the regular model performing better. An absence of arrows indicates comparable performance between the two models. We find that the average score of simple models tends to surpass regular models in most configurations.}
\label{tab:blimp_comp_contrastive_limited}
\end{table*}



==> tables/table_dataset_stats.tex <==
% dataset statistics

\begin{table}
\centering
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \textbf{Filtered} & \textbf{Unfiltered}\\
\midrule
PIQA & 795 & 1838 \\
ARC Easy & 339 & 2376 \\
Anaphor Agr. & 636 & 2000 \\
Argument Str. & 2603 & 9000 \\
Binding & 2296 & 7000 \\
Control/Raising & 1296 & 5000 \\
Determiner Noun Agr & 1691 & 7000 \\
Ellipsis & 416 & 2000 \\
Filler Gap & 1249 & 7000 \\
Irregular Forms & 979 & 2000 \\
Island Effects & 4132 & 8000 \\
NPI Lic. & 3714 & 7000 \\
Quantifiers & 2424 & 4000 \\
Subject Verb Agr. & 2099 & 6000 \\

\bottomrule

\end{tabular}
\caption{Number of samples used for different datasets. For each category in the BLiMP benchmark we sum the samples across the individual datasets in that particular category.}
\label{tab:stats_dataset}
\end{table}

==> tables/table_few_shot_filtered.tex <==
% few shot filtered
% \begin{table}
% \centering
% \begin{tabular}{lrrrrr}
% \toprule
%              Dataset &  0-shot &  1-shot &  2-shot &  3-shot &  4-shot \\
% \midrule
%      PIQA (filtered) &  0.6528 &  0.6428 &  0.6289 &  0.6277 &  0.6252 \\
%  ARC Easy (filtered) &  0.3982 &  0.3835 &  0.3835 &  0.3717 &  0.3628 \\
% \bottomrule
% \end{tabular}
% \caption{Few shot performance on PIQA and ARC Easy datasets. The evaluation is done on the biggest simple model with 1024 hidden size and 8 layers on the filtered dataset. We observe that few shot prompting does not improve model performance on models trained with simplified data.}
% \label{tab:few_shot}
% \end{table}

\begin{table}
\centering
\begin{tabular}{lrr}
\toprule
             Number of & PIQA  &  ARC Easy  \\
             Shots &  &  \\
\midrule
0 & 0.6528 & 0.3982 \\
1 & 0.6428 & 0.3835 \\
2 & 0.6289 & 0.3835 \\
3 & 0.6277 & 0.3717 \\
4 & 0.6252 & 0.3628 \\
\bottomrule
\end{tabular}
\caption{Few shot performance on PIQA and ARC Easy filtered datasets. The evaluation is done on the biggest simple model with 1024 hidden size and 8 layers on the filtered dataset. We observe that few shot prompting does not improve model performance on models trained with simplified data.}
\label{tab:few_shot}
\end{table}





==> tables/table_generalization.tex <==
% generalization results

\begin{table}[h!]
\centering
\begin{tabular}{llrrr}
\toprule
Hidden & Num. &  BLiMP &   PIQA &  ARC Easy \\
Size & Layers &   &    &  \\
\midrule
       1024 &           8 &  0.774 &  0.642 &     0.330 \\
       1024 &           4 &  0.748 &  0.627 &     0.310 \\
       1024 &           2 &  0.739 &  0.621 &     0.309 \\
        512 &           8 &  0.743 &  0.613 &     0.317 \\
        512 &           4 &  0.741 &  0.610 &     0.309 \\
        512 &           2 &  0.719 &  0.593 &     0.303 \\
        256 &           8 &  0.708 &  0.580 &     0.309 \\
        256 &           4 &  0.715 &  0.584 &     0.298 \\
        256 &           2 &  0.695 &  0.594 &     0.290 \\
        128 &           8 &  0.692 &  0.566 &     0.286 \\
        128 &           4 &  0.686 &  0.557 &     0.284 \\
        128 &           2 &  0.676 &  0.560 &     0.288 \\
         64 &           8 &  0.675 &  0.545 &     0.279 \\
         64 &           4 &  0.636 &  0.547 &     0.282 \\
         64 &           2 &  0.635 &  0.536 &     0.269 \\
         32 &           8 &  0.622 &  0.534 &     0.265 \\
         32 &           4 &  0.575 &  0.530 &     0.264 \\
         32 &           2 &  0.608 &  0.532 &     0.264 \\
\bottomrule
\end{tabular}
\caption{Zero-Shot accuracies of the simple model on the Unfiltered datasets. BLiMP denotes the average score on the BLiMP benchmark. We observe a deterioration of performance compared to the vocab-filtered datasets but we still see non-random performance.}
\label{tab:generalization}
\end{table}

